The Carina Project. V. The impact of NLTE effects on the iron content

We have performed accurate iron abundance measurements for 44 red giants (RGs) in the Carina dwarf spheroidal (dSph) galaxy. We used archival, high-resolution spectra (R~38,000) collected with UVES at ESO/VLT either in slit mode (5) or in fiber mode (39, FLAMES/GIRAFFE-UVES). The sample is more than a factor of four larger than any previous spectroscopic investigation of stars in dSphs based on high-resolution (R>38,000) spectra. We did not impose the ionization equilibrium between neutral and singly-ionized iron lines. The effective temperatures and the surface gravities were estimated by fitting stellar isochrones in the V, B-V color-magnitude diagram. To measure the iron abundance of individual lines we applied the LTE spectrum synthesis fitting method using MARCS model atmospheres of appropriate metallicity. We found evidence of NLTE effects between neutral and singly-ionized iron abundances. Assuming that the FeII abundances are minimally affected by NLTE effects, we corrected the FeI stellar abundances using a linear fit between FeI and FeII stellar abundance determinations. We found that the Carina metallicity distribution based on the corrected FeI abundances (44 RGs) has a weighted mean metallicity of [Fe/H]=-1.80 and a weighted standard deviation of sigma=0.24 dex. The Carina metallicity distribution based on the FeII abundances (27 RGs) gives similar estimates ([Fe/H]=-1.72, sigma=0.24 dex). The current weighted mean metallicities are slightly more metal poor when compared with similar estimates available in the literature. Furthermore, if we restrict our analysis to stars with the most accurate iron abundances, ~20 FeI and at least three FeII measurements (15 stars), we found that the range in iron abundances covered by Carina RGs (~1 dex) agrees quite well with similar estimates based on high-resolution spectra.

==> table2_complete.tex <==
\begin{deluxetable}{llllcccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccc}
\tabletypesize{\scriptsize}
\tablewidth{0pt}
\tablecaption{Atomic Data and Individual Iron Abundances}
\label{tab_lines_comp}
\tablehead{
\colhead{}&
\colhead{} &
\colhead{} &
\colhead{} &
	 \multicolumn{2}{c}{Car2} &
	 \multicolumn{2}{c}{Car3} &
	 \multicolumn{2}{c}{Car4} &
	 \multicolumn{2}{c}{Car10} &
	 \multicolumn{2}{c}{Car12} &
	 \multicolumn{2}{c}{Car13} &
	 \multicolumn{2}{c}{Car14} & 
	 \multicolumn{2}{c}{Car15} &
	 \multicolumn{2}{c}{Car16} &
	 \multicolumn{2}{c}{Car18} &
	 \multicolumn{2}{c}{Car19} &
	 \multicolumn{2}{c}{Car20} &
	 \multicolumn{2}{c}{Car21} &
	 \multicolumn{2}{c}{Car22} &
	 \multicolumn{2}{c}{Car23} &
	 \multicolumn{2}{c}{Car24} &
	 \multicolumn{2}{c}{Car25} &
	 \multicolumn{2}{c}{Car27} &
	 \multicolumn{2}{c}{Car28} &
	 \multicolumn{2}{c}{Car29} &
	 \multicolumn{2}{c}{Car30} &
	 \multicolumn{2}{c}{Car31} &
	 \multicolumn{2}{c}{Car32} &
	 \multicolumn{2}{c}{Car33} &
	 \multicolumn{2}{c}{Car34} &
	 \multicolumn{2}{c}{Car35} &
	 \multicolumn{2}{c}{Car36} &
	 \multicolumn{2}{c}{Car37} &
	 \multicolumn{2}{c}{Car38} &
	 \multicolumn{2}{c}{Car39} &
	 \multicolumn{2}{c}{Car40} &
	 \multicolumn{2}{c}{Car41} &
	 \multicolumn{2}{c}{Car42} &
	 \multicolumn{2}{c}{Car43} &
	 \multicolumn{2}{c}{Car44} &
	 \multicolumn{2}{c}{Car45} &
	 \multicolumn{2}{c}{Car46} &
	 \multicolumn{2}{c}{Car47} &
	 \multicolumn{2}{c}{Car48} &
	 \multicolumn{2}{c}{Car49} &
	 \multicolumn{2}{c}{Car50} & 
	 \multicolumn{2}{c}{Car51} &
	 \multicolumn{2}{c}{Car52} &
	 \multicolumn{2}{c}{Car53} \\
\colhead{$\lambda$ (\AA)}&
\colhead{Elem.} &
\colhead{EP (eV)} &
\colhead{$\log gf$} &
 \colhead{\feh} & \colhead{EW\tablenotemark{a}} &
 \colhead{\feh} & \colhead{EW\tablenotemark{a}} &
 \colhead{\feh} & \colhead{EW\tablenotemark{a}} &
 \colhead{\feh} & \colhead{EW\tablenotemark{a}} &
 \colhead{\feh} & \colhead{EW\tablenotemark{a}} &
 \colhead{\feh} & \colhead{EW\tablenotemark{a}} &
 \colhead{\feh} & \colhead{EW\tablenotemark{a}} &
 \colhead{\feh} & \colhead{EW\tablenotemark{a}} &
 \colhead{\feh} & \colhead{EW\tablenotemark{a}} &
 \colhead{\feh} & \colhead{EW\tablenotemark{a}} &
 \colhead{\feh} & \colhead{EW\tablenotemark{a}} &
 \colhead{\feh} & \colhead{EW\tablenotemark{a}} &
 \colhead{\feh} & \colhead{EW\tablenotemark{a}} &
 \colhead{\feh} & \colhead{EW\tablenotemark{a}} &
 \colhead{\feh} & \colhead{EW\tablenotemark{a}} &
 \colhead{\feh} & \colhead{EW\tablenotemark{a}} &
 \colhead{\feh} & \colhead{EW\tablenotemark{a}} &
 \colhead{\feh} & \colhead{EW\tablenotemark{a}} &
 \colhead{\feh} & \colhead{EW\tablenotemark{a}} &
 \colhead{\feh} & \colhead{EW\tablenotemark{a}} &
 \colhead{\feh} & \colhead{EW\tablenotemark{a}} &
 \colhead{\feh} & \colhead{EW\tablenotemark{a}} &
 \colhead{\feh} & \colhead{EW\tablenotemark{a}} &
 \colhead{\feh} & \colhead{EW\tablenotemark{a}} &
 \colhead{\feh} & \colhead{EW\tablenotemark{a}} &
 \colhead{\feh} & \colhead{EW\tablenotemark{a}} &
 \colhead{\feh} & \colhead{EW\tablenotemark{a}} &
 \colhead{\feh} & \colhead{EW\tablenotemark{a}} &
 \colhead{\feh} & \colhead{EW\tablenotemark{a}} &
 \colhead{\feh} & \colhead{EW\tablenotemark{a}} &
 \colhead{\feh} & \colhead{EW\tablenotemark{a}} &
 \colhead{\feh} & \colhead{EW\tablenotemark{a}} &
 \colhead{\feh} & \colhead{EW\tablenotemark{a}} &
 \colhead{\feh} & \colhead{EW\tablenotemark{a}} &
 \colhead{\feh} & \colhead{EW\tablenotemark{a}} &
 \colhead{\feh} & \colhead{EW\tablenotemark{a}} &
 \colhead{\feh} & \colhead{EW\tablenotemark{a}} &
 \colhead{\feh} & \colhead{EW\tablenotemark{a}} &
 \colhead{\feh} & \colhead{EW\tablenotemark{a}} &
 \colhead{\feh} & \colhead{EW\tablenotemark{a}} &
 \colhead{\feh} & \colhead{EW\tablenotemark{a}} &
 \colhead{\feh} & \colhead{EW\tablenotemark{a}} &
 \colhead{\feh} & \colhead{EW\tablenotemark{a}} &
 \colhead{\feh} & \colhead{EW\tablenotemark{a}} &
 } 
\startdata
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
4924.770& 26.0& 2.279&$ -2.241$ & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.55\pm0.16$ &   69. & \ldots & \ldots \\
4950.110& 26.0& 3.417&$ -1.670$ & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.75\pm0.14$ &   55. & \ldots & \ldots & \ldots & \ldots &$-1.75\pm0.16$ &   49. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.70\pm0.16$ &   62. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.05\pm0.15$ &   43. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.65\pm0.14$ &   75. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.05\pm0.13$ &   34. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
4973.100& 26.0& 3.960&$ -0.950$ & \ldots & \ldots &$-2.20\pm0.14$ &   88. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.05\pm0.14$ &   42. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.70\pm0.14$ &   87. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.75\pm0.18$ &   89.\\
5044.210& 26.0& 2.851&$ -2.038$ & \ldots & \ldots &$-2.15\pm0.13$ &   93. & \ldots & \ldots &$-2.10\pm0.12$ &   51. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.95\pm0.15$ &   56. & \ldots & \ldots & \ldots & \ldots &$-2.05\pm0.15$ &   78. &$-1.95\pm0.15$ &   61. &$-2.20\pm0.14$ &   58. & \ldots & \ldots &$-2.05\pm0.15$ &   63. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.15\pm0.13$ &   68. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.95\pm0.16$ &   56. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.05\pm0.16$ &   38. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
5054.640& 26.0& 3.640&$ -1.921$ & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.45\pm0.16$ &   31. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.70\pm0.15$ &   28. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
5090.770& 26.0& 4.256&$ -0.400$ & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.95\pm0.13$ &   49. &$-2.25\pm0.13$ &   36. & \ldots & \ldots & \ldots & \ldots &$-2.15\pm0.12$ &   30. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.10\pm0.15$ &   63. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
5197.580& 26.1& 3.230&$ -2.348$ &$-1.55\pm0.30$ &  105. &$-1.85\pm0.38$ &  117. &$-1.49\pm0.42$ &  104. &$-2.00\pm0.21$ &   73. &$-1.45\pm0.29$ &   89. & \ldots & \ldots &$-1.60\pm0.23$ &   94. &$-1.99\pm0.34$ &   92. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.45\pm0.27$ &   89. & \ldots & \ldots &$-1.95\pm0.43$ &   50. &$-1.65\pm0.28$ &   93. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.80\pm0.25$ &   79. & \ldots & \ldots &$-2.05\pm0.53$ &   58. & \ldots & \ldots & \ldots & \ldots &$-2.00\pm0.27$ &   77. &$-1.63\pm0.50$ &   82. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.65\pm0.29$ &   81.\\
5215.180& 26.0& 3.266&$ -0.871$ & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.80\pm0.13$ &   49. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
5217.390& 26.0& 3.211&$ -1.070$ & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.90\pm0.13$ &   45. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.60\pm0.14$ &   29. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
5234.620& 26.1& 3.221&$ -2.279$ & \ldots & \ldots &$-1.95\pm0.34$ &   83. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.63\pm0.36$ &   92. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.30\pm0.26$ &  110. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.95\pm0.23$ &   69. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.68\pm0.41$ &   86. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.90\pm0.27$ &   77. & \ldots & \ldots & \ldots & \ldots &$-2.30\pm0.22$ &   47. & \ldots & \ldots &$-1.75\pm0.28$ &  105. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
5242.490& 26.0& 3.634&$ -0.967$ & \ldots & \ldots &$-2.05\pm0.17$ &   98. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.35\pm0.19$ &   48. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.20\pm0.13$ &   39. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
5264.810& 26.1& 3.230&$ -3.133$ & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.30\pm0.29$ &   46. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.25\pm0.30$ &   74. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.40\pm0.31$ &   92. & \ldots & \ldots & \ldots & \ldots \\
5284.110& 26.1& 2.891&$ -3.195$ & \ldots & \ldots & \ldots & \ldots &$-1.55\pm0.20$ &   65. & \ldots & \ldots &$-1.45\pm0.23$ &   46. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.55\pm1.30$ &   92. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
5288.520& 26.0& 3.694&$ -1.508$ &$-1.65\pm0.13$ &   52. & \ldots & \ldots &$-1.70\pm0.24$ &   56. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.79\pm0.20$ &   42. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
5307.360& 26.0& 1.608&$ -2.987$ & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.75\pm0.12$ &   51. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.45\pm0.13$ &   45. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.85\pm0.13$ &   49. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.65\pm0.13$ &   44. &$-2.55\pm0.13$ &   41. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
5316.620& 26.1& 3.153&$ -2.014$ & \ldots & \ldots &$-2.05\pm0.20$ &  156. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.95\pm0.20$ &   88. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.10\pm0.15$ &  137. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
5362.870& 26.1& 3.199&$ -2.616$ &$-1.55\pm0.21$ &   83. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.65\pm0.16$ &   85. & \ldots & \ldots & \ldots & \ldots &$-1.75\pm0.23$ &   67. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.45\pm0.23$ &  104. & \ldots & \ldots &$-1.95\pm0.19$ &   59. &$-1.65\pm0.17$ &   90. & \ldots & \ldots &$-1.85\pm0.21$ &   83. &$-2.00\pm0.22$ &   50. & \ldots & \ldots & \ldots & \ldots &$-1.80\pm0.17$ &   96. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.60\pm0.15$ &   88. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.95\pm0.23$ &   42. & \ldots & \ldots &$-1.90\pm0.24$ &   51. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.95\pm0.22$ &   42. & \ldots & \ldots & \ldots & \ldots &$-1.50\pm0.27$ &   86. & \ldots & \ldots &$-1.85\pm0.25$ &   62.\\
5364.870& 26.0& 4.445&$  0.228$ & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.35\pm0.12$ &   57. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
5365.400& 26.0& 3.573&$ -1.020$ & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.15\pm0.13$ &   57. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
5367.470& 26.0& 4.415&$  0.443$ & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.85\pm0.12$ &   38. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
5369.960& 26.0& 4.370&$  0.540$ & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.90\pm0.12$ &   49. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
5391.460& 26.0& 4.154&$ -0.782$ & \ldots & \ldots &$-2.25\pm0.13$ &   55. & \ldots & \ldots & \ldots & \ldots &$-1.70\pm0.14$ &   69. & \ldots & \ldots &$-1.70\pm0.13$ &   80. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.05\pm0.14$ &   48. & \ldots & \ldots & \ldots & \ldots &$-1.85\pm0.13$ &   49. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
5398.280& 26.0& 4.445&$ -0.670$ & \ldots & \ldots &$-2.05\pm0.13$ &   33. & \ldots & \ldots & \ldots & \ldots &$-1.55\pm0.14$ &   66. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.50\pm0.13$ &   54. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.55\pm0.15$ &   95. & \ldots & \ldots & \ldots & \ldots \\
5445.040& 26.0& 4.386&$ -0.020$ & \ldots & \ldots &$-2.25\pm0.28$ &   72. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.20\pm0.12$ &   57. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.20\pm0.12$ &   44. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
5466.400& 26.0& 4.371&$ -0.630$ & \ldots & \ldots &$-2.15\pm0.28$ &   46. & \ldots & \ldots & \ldots & \ldots &$-1.75\pm0.13$ &   50. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.00\pm0.13$ &   37. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.75\pm0.14$ &   57. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
5534.850& 26.1& 3.245&$ -2.865$ &$-1.45\pm0.17$ &   59. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.50\pm0.18$ &   73. & \ldots & \ldots &$-1.70\pm0.15$ &   61. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.25\pm0.14$ &   92. & \ldots & \ldots & \ldots & \ldots &$-1.50\pm0.20$ &   75. &$-1.60\pm0.17$ &   58. &$-1.75\pm0.17$ &   61. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.70\pm0.16$ &   54. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.65\pm0.19$ &   72.\\
5554.890& 26.0& 4.548&$ -0.440$ &$-1.65\pm0.12$ &   52. & \ldots & \ldots &$-1.55\pm0.12$ &   67. & \ldots & \ldots &$-1.60\pm0.12$ &   48. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.75\pm0.12$ &   61. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.85\pm0.12$ &   37. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.70\pm0.12$ &   53. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
5576.090& 26.0& 3.430&$ -1.000$ & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.75\pm0.12$ &   32. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.35\pm0.13$ &   41. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
5633.950& 26.0& 4.991&$ -0.270$ & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.45\pm0.12$ &   48. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
5638.260& 26.0& 4.220&$ -0.870$ & \ldots & \ldots &$-2.15\pm0.13$ &   40. & \ldots & \ldots &$-1.95\pm0.13$ &   22. &$-1.65\pm0.12$ &   49. & \ldots & \ldots &$-1.65\pm0.12$ &   50. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.65\pm0.12$ &   59. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.65\pm0.12$ &   47. & \ldots & \ldots &$-1.70\pm0.12$ &   54. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.80\pm0.13$ &   52. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
5859.590& 26.0& 4.549&$ -0.419$ &$-1.70\pm0.12$ &   50. &$-2.20\pm0.12$ &   38. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.70\pm0.12$ &   53. & \ldots & \ldots & \ldots & \ldots &$-1.65\pm0.13$ &   62. & \ldots & \ldots & \ldots & \ldots &$-1.90\pm0.12$ &   28. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.85\pm0.12$ &   47. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.05\pm0.13$ &   43.\\
5862.360& 26.0& 4.549&$ -0.127$ & \ldots & \ldots &$-2.20\pm0.12$ &   52. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.95\pm0.12$ &   59. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.05\pm0.12$ &   60. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.05\pm0.12$ &   52. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
5916.250& 26.0& 2.453&$ -2.994$ & \ldots & \ldots &$-2.20\pm0.12$ &   50. &$-1.65\pm0.12$ &   90. & \ldots & \ldots &$-1.85\pm0.13$ &   58. & \ldots & \ldots &$-1.70\pm0.12$ &   65. &$-2.20\pm0.12$ &   44. & \ldots & \ldots & \ldots & \ldots &$-1.65\pm0.12$ &   81. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.75\pm0.13$ &   57. &$-1.90\pm0.12$ &   58. &$-2.05\pm0.12$ &   40. & \ldots & \ldots &$-1.55\pm0.12$ &   80. & \ldots & \ldots &$-1.65\pm0.12$ &   89. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.90\pm0.14$ &   54. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.10\pm0.12$ &   47. &$-1.55\pm0.15$ &   79. & \ldots & \ldots &$-1.70\pm0.13$ &   57.\\
5930.180& 26.0& 4.652&$ -0.230$ & \ldots & \ldots &$-2.05\pm0.12$ &   49. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.80\pm0.12$ &   49. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.85\pm0.12$ &   43. & \ldots & \ldots &$-1.85\pm0.12$ &   50. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.95\pm0.12$ &   43. &$-2.00\pm0.12$ &   40. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.70\pm0.12$ &   66. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
5934.650& 26.0& 3.928&$ -1.170$ &$-1.60\pm0.14$ &   68. & \ldots & \ldots &$-1.65\pm0.12$ &   72. & \ldots & \ldots &$-1.80\pm0.13$ &   40. & \ldots & \ldots &$-1.80\pm0.12$ &   50. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.85\pm0.12$ &   38. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.95\pm0.12$ &   53. &$-2.10\pm0.12$ &   31. & \ldots & \ldots &$-1.75\pm0.12$ &   48. & \ldots & \ldots &$-1.70\pm0.12$ &   70. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.90\pm0.14$ &   31. &$-2.15\pm0.12$ &   27. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
5952.720& 26.0& 3.984&$ -1.440$ & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.45\pm0.12$ &   60. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.60\pm0.17$ &   57. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
5956.690& 26.0& 0.859&$ -4.605$ & \ldots & \ldots &$-2.20\pm0.16$ &  127. & \ldots & \ldots &$-2.10\pm0.12$ &   85. & \ldots & \ldots & \ldots & \ldots &$-1.95\pm0.12$ &  102. &$-2.22\pm0.16$ &   95. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.80\pm0.12$ &   95. & \ldots & \ldots &$-1.95\pm0.13$ &   97. &$-2.10\pm0.12$ &   49. &$-2.15\pm0.13$ &   97. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.20\pm0.12$ &   87. &$-2.05\pm0.12$ &   82. & \ldots & \ldots & \ldots & \ldots &$-2.18\pm0.17$ &   62. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.35\pm0.12$ &   75. & \ldots & \ldots & \ldots & \ldots &$-1.85\pm0.13$ &   93. & \ldots & \ldots &$-2.23\pm0.17$ &   78. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
5976.780& 26.0& 3.943&$ -1.243$ & \ldots & \ldots & \ldots & \ldots &$-1.70\pm0.12$ &   54. & \ldots & \ldots &$-1.80\pm0.12$ &   42. & \ldots & \ldots &$-1.75\pm0.12$ &   47. & \ldots & \ldots & \ldots & \ldots &$-1.85\pm0.13$ &   37. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.50\pm0.13$ &   68. & \ldots & \ldots & \ldots & \ldots &$-1.80\pm0.13$ &   48. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.80\pm0.12$ &   35. &$-1.95\pm0.12$ &   41. &$-2.10\pm0.12$ &   30. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.15\pm0.12$ &   38. & \ldots & \ldots & \ldots & \ldots &$-1.80\pm0.13$ &   52.\\
5984.810& 26.0& 4.733&$ -0.196$ & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.85\pm0.12$ &   42. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.85\pm0.12$ &   32. &$-1.80\pm0.13$ &   52. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.80\pm0.12$ &   44. & \ldots & \ldots &$-2.10\pm0.12$ &   26. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.15\pm0.12$ &   39. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
6003.010& 26.0& 3.881&$ -1.120$ & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.85\pm0.12$ &   63. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.95\pm0.12$ &   24. &$-1.90\pm0.13$ &   65. &$-2.15\pm0.12$ &   21. &$-2.05\pm0.13$ &   49. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.85\pm0.12$ &   49. &$-2.05\pm0.12$ &   39. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.70\pm0.12$ &   74. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.95\pm0.12$ &   50. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
6008.560& 26.0& 3.884&$ -0.986$ & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.95\pm0.12$ &   27. &$-1.92\pm0.17$ &   77. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.95\pm0.12$ &   35. & \ldots & \ldots &$-2.10\pm0.12$ &   29. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.05\pm0.12$ &   55. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
6012.210& 26.0& 2.223&$ -4.038$ & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.30\pm0.12$ &   58. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
6020.170& 26.0& 4.607&$ -0.270$ & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.80\pm0.13$ &   78. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
6024.060& 26.0& 4.548&$ -0.120$ & \ldots & \ldots &$-2.06\pm0.20$ &   81. & \ldots & \ldots &$-2.15\pm0.12$ &   43. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.95\pm0.12$ &   65. & \ldots & \ldots & \ldots & \ldots &$-2.05\pm0.12$ &   42. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.20\pm0.15$ &   37. & \ldots & \ldots & \ldots & \ldots &$-2.00\pm0.13$ &   44.\\
6027.050& 26.0& 4.076&$ -1.089$ & \ldots & \ldots &$-2.20\pm0.12$ &   58. &$-1.60\pm0.12$ &   63. & \ldots & \ldots &$-1.55\pm0.12$ &   59. & \ldots & \ldots &$-1.75\pm0.12$ &   44. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.05\pm0.12$ &   29. & \ldots & \ldots &$-1.65\pm0.12$ &   53. & \ldots & \ldots &$-1.70\pm0.12$ &   58. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.15\pm0.15$ &   32. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
6056.000& 26.0& 4.733&$ -0.460$ & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.45\pm0.12$ &   64. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.70\pm0.12$ &   44. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
6065.480& 26.0& 2.608&$ -1.530$ & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.95\pm0.12$ &   52. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
6082.710& 26.0& 2.223&$ -3.573$ & \ldots & \ldots &$-2.05\pm0.12$ &   49. &$-1.75\pm0.13$ &   49. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.75\pm0.12$ &   48. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.55\pm0.12$ &   73. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.85\pm0.12$ &   40. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.65\pm0.12$ &   50. & \ldots & \ldots &$-1.75\pm0.12$ &   64. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.10\pm0.12$ &   33. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
6085.260& 26.0& 2.758&$ -3.095$ & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.50\pm0.12$ &   59. & \ldots & \ldots & \ldots & \ldots &$-1.25\pm0.13$ &   84. &$-1.60\pm0.12$ &   47. & \ldots & \ldots &$-1.65\pm0.12$ &   62. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
6136.990& 26.0& 2.198&$ -2.950$ & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.25\pm0.16$ &   69. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.05\pm0.12$ &   55. &$-2.05\pm0.14$ &   88. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
6151.620& 26.0& 2.176&$ -3.299$ &$-1.65\pm0.13$ &   86. &$-2.20\pm0.13$ &   91. & \ldots & \ldots & \ldots & \ldots &$-1.55\pm0.14$ &   87. & \ldots & \ldots &$-1.80\pm0.12$ &   61. &$-2.20\pm0.12$ &   38. &$-1.65\pm0.14$ &   70. &$-1.80\pm0.13$ &   70. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.70\pm0.13$ &   63. & \ldots & \ldots &$-1.75\pm0.12$ &   66. & \ldots & \ldots &$-2.05\pm0.14$ &   51. & \ldots & \ldots & \ldots & \ldots &$-1.75\pm0.13$ &   60. &$-1.90\pm0.12$ &   56. &$-1.95\pm0.13$ &   46. & \ldots & \ldots &$-1.70\pm0.13$ &   76. & \ldots & \ldots &$-1.75\pm0.12$ &   87. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.70\pm0.14$ &   61. &$-1.75\pm0.14$ &   56. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
6157.730& 26.0& 4.076&$ -1.260$ & \ldots & \ldots &$-2.05\pm0.13$ &   40. &$-1.65\pm0.13$ &   48. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.55\pm0.12$ &   58. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.65\pm0.13$ &   37. & \ldots & \ldots &$-1.70\pm0.12$ &   46. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.60\pm0.13$ &   50. & \ldots & \ldots &$-1.55\pm0.12$ &   62. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.50\pm0.14$ &   56. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
6170.510& 26.0& 4.795&$ -0.440$ &$-1.65\pm0.13$ &   49. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.55\pm0.14$ &   52. & \ldots & \ldots &$-1.80\pm0.12$ &   47. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.55\pm0.12$ &   56. & \ldots & \ldots & \ldots & \ldots &$-1.45\pm0.14$ &   79. &$-1.60\pm0.13$ &   56. & \ldots & \ldots &$-1.70\pm0.12$ &   48. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
6173.330& 26.0& 2.223&$ -2.880$ & \ldots & \ldots &$-2.20\pm0.13$ &  104. & \ldots & \ldots &$-2.10\pm0.13$ &   61. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.25\pm0.12$ &   69. &$-1.95\pm0.14$ &   78. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.95\pm0.13$ &   40. & \ldots & \ldots & \ldots & \ldots &$-2.05\pm0.14$ &   94. & \ldots & \ldots &$-2.30\pm0.13$ &   35. &$-1.95\pm0.13$ &   70. &$-1.95\pm0.12$ &   81. &$-2.10\pm0.13$ &   67. &$-2.00\pm0.15$ &   52. & \ldots & \ldots &$-2.15\pm0.12$ &   49. & \ldots & \ldots & \ldots & \ldots &$-1.95\pm0.16$ &  102. & \ldots & \ldots &$-1.95\pm0.15$ &   75. & \ldots & \ldots &$-1.90\pm0.14$ &   53. & \ldots & \ldots & \ldots & \ldots &$-2.20\pm0.13$ &   36. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.10\pm0.13$ &   81. & \ldots & \ldots & \ldots & \ldots &$-2.00\pm0.14$ &   78.\\
6180.200& 26.0& 2.727&$ -2.586$ &$-1.70\pm0.13$ &   70. &$-2.20\pm0.13$ &   64. &$-1.70\pm0.13$ &   80. & \ldots & \ldots &$-1.65\pm0.14$ &   65. & \ldots & \ldots &$-1.85\pm0.12$ &   62. &$-2.35\pm0.12$ &   40. & \ldots & \ldots & \ldots & \ldots &$-1.60\pm0.12$ &   79. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.15\pm0.14$ &   38. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.10\pm0.12$ &   50. &$-2.05\pm0.13$ &   49. &$-1.95\pm0.15$ &   33. &$-1.80\pm0.13$ &   55. & \ldots & \ldots &$-1.85\pm0.12$ &   72. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.10\pm0.13$ &   43. & \ldots & \ldots & \ldots & \ldots &$-1.95\pm0.14$ &   43.\\
6187.990& 26.0& 3.943&$ -1.720$ & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.45\pm0.14$ &   35. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.25\pm0.14$ &   46. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
6200.310& 26.0& 2.608&$ -2.437$ & \ldots & \ldots &$-2.05\pm0.12$ &   97. & \ldots & \ldots &$-1.95\pm0.13$ &   65. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.20\pm0.12$ &   54. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.15\pm0.12$ &   43. & \ldots & \ldots &$-1.95\pm0.13$ &   71. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.00\pm0.12$ &   62. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.15\pm0.13$ &   70. & \ldots & \ldots & \ldots & \ldots &$-1.95\pm0.14$ &   77.\\
6213.430& 26.0& 2.223&$ -2.482$ & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.65\pm0.12$ &   33. & \ldots & \ldots &$-2.35\pm0.12$ &   90. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.65\pm0.13$ &   29. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.35\pm0.13$ &   53. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.30\pm0.15$ &   51. & \ldots & \ldots \\
6219.280& 26.0& 2.198&$ -2.433$ & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.70\pm0.12$ &   44. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.40\pm0.13$ &   69. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.60\pm0.14$ &   65. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
6240.650& 26.0& 2.223&$ -3.233$ &$-1.65\pm0.15$ &   96. &$-2.20\pm0.12$ &   52. &$-1.70\pm0.12$ &   72. & \ldots & \ldots &$-1.65\pm0.13$ &   79. & \ldots & \ldots &$-1.80\pm0.13$ &   69. &$-2.30\pm0.12$ &   36. & \ldots & \ldots & \ldots & \ldots &$-1.55\pm0.12$ &   96. & \ldots & \ldots & \ldots & \ldots &$-1.55\pm0.13$ &  101. &$-1.75\pm0.13$ &   65. & \ldots & \ldots &$-1.90\pm0.13$ &   57. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.95\pm0.13$ &   43. &$-1.95\pm0.13$ &   59. &$-2.05\pm0.12$ &   48. & \ldots & \ldots &$-1.75\pm0.13$ &   63. & \ldots & \ldots &$-1.75\pm0.12$ &   85. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.10\pm0.13$ &   46. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
6246.320& 26.0& 3.602&$ -0.733$ & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.95\pm0.12$ &   23. & \ldots & \ldots &$-2.45\pm0.12$ &   62. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
6247.560& 26.1& 3.892&$ -2.435$ &$-1.45\pm0.28$ &   49. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.40\pm0.22$ &   53. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.30\pm0.18$ &   61. & \ldots & \ldots & \ldots & \ldots &$-1.35\pm0.21$ &   67. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
6254.260& 26.0& 2.279&$ -2.443$ & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.88\pm0.18$ &   57. & \ldots & \ldots &$-2.30\pm0.17$ &   92. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.45\pm0.13$ &   67. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
6265.130& 26.0& 2.176&$ -2.550$ & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.73\pm0.18$ &   49. & \ldots & \ldots &$-2.30\pm0.17$ &   95. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.45\pm0.17$ &   68. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
6270.220& 26.0& 2.858&$ -2.464$ &$-1.75\pm0.14$ &   93. & \ldots & \ldots &$-1.70\pm0.12$ &   76. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.85\pm0.13$ &   51. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.65\pm0.13$ &   79. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.70\pm0.20$ &   61. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.95\pm0.13$ &   47. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.85\pm0.13$ &   72. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.75\pm0.13$ &   62. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
6318.020& 26.0& 2.453&$ -2.261$ & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.45\pm0.13$ &   54. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.45\pm0.28$ &   49. & \ldots & \ldots &$-2.45\pm0.17$ &   59. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
6322.690& 26.0& 2.588&$ -2.426$ & \ldots & \ldots &$-2.25\pm0.13$ &   97. & \ldots & \ldots &$-2.10\pm0.12$ &   62. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.29\pm0.18$ &   65. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.98\pm0.19$ &   92. &$-1.95\pm0.13$ &   75. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.95\pm0.20$ &   69. & \ldots & \ldots &$-2.02\pm0.19$ &   87. & \ldots & \ldots & \ldots & \ldots &$-2.12\pm0.19$ &   55. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.95\pm0.24$ &   41. & \ldots & \ldots &$-2.15\pm0.18$ &   68. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
6335.330& 26.0& 2.198&$ -2.177$ & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.80\pm0.13$ &   63. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
6336.820& 26.0& 3.686&$ -0.856$ & \ldots & \ldots &$-2.20\pm0.12$ &  115. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.45\pm0.12$ &   50. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.35\pm0.13$ &   50. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.25\pm0.13$ &   46. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
6355.030& 26.0& 2.845&$ -2.350$ & \ldots & \ldots &$-2.20\pm0.12$ &   82. & \ldots & \ldots &$-2.05\pm0.12$ &   39. & \ldots & \ldots & \ldots & \ldots &$-1.80\pm0.12$ &   89. &$-2.20\pm0.12$ &   44. & \ldots & \ldots &$-1.85\pm0.15$ &   66. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.85\pm0.13$ &   76. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.10\pm0.13$ &   19. &$-1.80\pm0.13$ &   70. &$-1.85\pm0.12$ &   65. &$-2.00\pm0.12$ &   53. & \ldots & \ldots & \ldots & \ldots &$-2.15\pm0.13$ &   35. &$-1.70\pm0.12$ &   95. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.95\pm0.13$ &   53. & \ldots & \ldots & \ldots & \ldots &$-1.85\pm0.14$ &   60.\\
6408.020& 26.0& 3.686&$ -1.018$ & \ldots & \ldots &$-2.20\pm0.12$ &   82. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.40\pm0.12$ &   44. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.25\pm0.12$ &   34. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.15\pm0.12$ &   57. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
6411.650& 26.0& 3.654&$ -0.595$ & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.95\pm0.12$ &   43. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
6419.950& 26.0& 4.733&$ -0.240$ & \ldots & \ldots &$-2.05\pm0.12$ &   40. &$-1.65\pm0.12$ &   52. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.95\pm0.12$ &   39. & \ldots & \ldots & \ldots & \ldots &$-1.70\pm0.12$ &   51. & \ldots & \ldots &$-1.75\pm0.12$ &   55. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
6421.350& 26.0& 2.279&$ -2.027$ & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.80\pm0.12$ &   65. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.70\pm0.13$ &   75. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
6432.680& 26.1& 2.891&$ -3.687$ & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.35\pm0.21$ &   61. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.25\pm0.15$ &   59. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
6456.380& 26.1& 3.903&$ -2.185$ &$-1.65\pm0.26$ &   45. & \ldots & \ldots &$-1.60\pm0.28$ &   39. & \ldots & \ldots &$-1.45\pm0.21$ &   65. & \ldots & \ldots &$-1.65\pm0.28$ &   55. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.29\pm0.27$ &   87. & \ldots & \ldots & \ldots & \ldots &$-1.45\pm0.19$ &   71. & \ldots & \ldots & \ldots & \ldots &$-1.70\pm0.16$ &   53. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.70\pm0.23$ &   41. & \ldots & \ldots & \ldots & \ldots &$-1.65\pm0.21$ &   59. & \ldots & \ldots &$-1.61\pm0.28$ &   57. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
6475.620& 26.0& 2.559&$ -2.942$ &$-1.65\pm0.15$ &   77. &$-2.05\pm0.14$ &   83. &$-1.55\pm0.14$ &   97. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.70\pm0.14$ &   70. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.50\pm0.14$ &   96. &$-1.60\pm0.13$ &   67. & \ldots & \ldots &$-1.80\pm0.14$ &   71. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.85\pm0.14$ &   56. &$-1.80\pm0.13$ &   61. & \ldots & \ldots &$-1.60\pm0.13$ &   87. &$-2.05\pm0.12$ &   36. &$-1.65\pm0.14$ &   90. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.60\pm0.14$ &   53. & \ldots & \ldots &$-1.70\pm0.14$ &   69.\\
6481.870& 26.0& 2.279&$ -2.984$ & \ldots & \ldots &$-2.20\pm0.14$ &   95. & \ldots & \ldots &$-2.10\pm0.13$ &   49. & \ldots & \ldots & \ldots & \ldots &$-1.80\pm0.14$ &   79. &$-2.20\pm0.12$ &   65. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.80\pm0.15$ &   73. &$-1.80\pm0.17$ &  104. & \ldots & \ldots & \ldots & \ldots &$-1.90\pm0.14$ &   61. &$-1.90\pm0.14$ &   93. &$-1.95\pm0.13$ &   59. &$-1.85\pm0.13$ &   81. & \ldots & \ldots &$-2.00\pm0.13$ &   55. &$-1.80\pm0.14$ &   81. &$-1.85\pm0.14$ &   76. &$-1.85\pm0.13$ &   76. & \ldots & \ldots & \ldots & \ldots &$-2.10\pm0.12$ &   46. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.80\pm0.15$ &   60. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.75\pm0.17$ &   59. &$-1.80\pm0.16$ &   76. & \ldots & \ldots &$-2.20\pm0.14$ &   49. & \ldots & \ldots &$-2.05\pm0.14$ &   44. &$-1.75\pm0.14$ &   76.\\
6498.940& 26.0& 0.958&$ -4.699$ &$-1.60\pm0.15$ &  121. &$-2.20\pm0.14$ &  109. &$-1.65\pm0.14$ &  118. &$-2.15\pm0.13$ &   58. &$-1.55\pm0.14$ &  125. & \ldots & \ldots &$-1.75\pm0.14$ &  108. &$-2.30\pm0.12$ &   69. &$-1.70\pm0.14$ &  101. &$-1.75\pm0.15$ &   94. &$-1.70\pm0.13$ &  117. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.75\pm0.13$ &  100. &$-1.75\pm0.14$ &   51. &$-1.90\pm0.14$ &   93. &$-2.00\pm0.13$ &   51. &$-1.95\pm0.14$ &   79. &$-1.95\pm0.17$ &   65. &$-2.05\pm0.13$ &   47. &$-1.90\pm0.14$ &   80. &$-1.90\pm0.14$ &   85. &$-2.00\pm0.13$ &   89. & \ldots & \ldots &$-1.55\pm0.13$ &  127. &$-2.10\pm0.12$ &   55. &$-1.70\pm0.14$ &  131. & \ldots & \ldots &$-1.65\pm0.16$ &   92. & \ldots & \ldots &$-1.80\pm0.15$ &   84. &$-1.70\pm0.15$ &   70. &$-1.75\pm0.15$ &   78. & \ldots & \ldots &$-2.40\pm0.14$ &   39. & \ldots & \ldots & \ldots & \ldots &$-1.75\pm0.16$ &   83. &$-1.80\pm0.15$ &   95. &$-2.15\pm0.14$ &   70. & \ldots & \ldots & \ldots & \ldots &$-1.95\pm0.14$ &   83.\\
6516.080& 26.1& 2.891&$ -3.432$ &$-1.65\pm0.26$ &   48. & \ldots & \ldots &$-1.60\pm0.24$ &   51. & \ldots & \ldots &$-1.45\pm0.23$ &   64. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.60\pm0.27$ &   47. &$-1.30\pm0.22$ &   75. & \ldots & \ldots & \ldots & \ldots &$-1.50\pm0.23$ &   59. &$-1.55\pm0.20$ &   58. &$-1.65\pm0.24$ &   52. &$-1.65\pm0.23$ &   62. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.65\pm0.24$ &   51. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.50\pm0.25$ &   52. & \ldots & \ldots & \ldots & \ldots \\
6518.370& 26.0& 2.831&$ -2.460$ &$-1.65\pm0.15$ &   80. &$-2.25\pm0.14$ &   61. &$-1.70\pm0.14$ &   85. & \ldots & \ldots &$-1.65\pm0.14$ &   76. & \ldots & \ldots &$-1.85\pm0.14$ &   59. &$-2.25\pm0.12$ &   39. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.70\pm0.13$ &   70. & \ldots & \ldots &$-1.80\pm0.14$ &   64. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.10\pm0.14$ &   50. &$-1.95\pm0.13$ &   54. & \ldots & \ldots & \ldots & \ldots &$-2.10\pm0.12$ &   35. &$-1.75\pm0.14$ &   88. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.15\pm0.14$ &   51. & \ldots & \ldots & \ldots & \ldots &$-1.85\pm0.14$ &   53.\\
6546.240& 26.0& 2.758&$ -1.536$ & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.90\pm0.22$ &   50. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
6569.210& 26.0& 4.733&$ -0.420$ &$-1.55\pm0.18$ &   52. & \ldots & \ldots &$-1.60\pm0.18$ &   55. & \ldots & \ldots &$-1.50\pm0.27$ &   67. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.50\pm0.23$ &   58. & \ldots & \ldots & \ldots & \ldots &$-1.55\pm0.31$ &   63. &$-1.70\pm0.26$ &   47. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.65\pm0.25$ &   64. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
6574.230& 26.0& 0.990&$ -5.023$ &$-1.60\pm0.18$ &   91. &$-2.20\pm0.18$ &   81. &$-1.65\pm0.18$ &   97. &$-2.10\pm0.18$ &   32. &$-1.40\pm0.27$ &  107. & \ldots & \ldots &$-1.70\pm0.30$ &   80. &$-2.30\pm0.17$ &   36. & \ldots & \ldots & \ldots & \ldots &$-1.50\pm0.23$ &   87. & \ldots & \ldots & \ldots & \ldots &$-1.40\pm0.31$ &  114. &$-1.60\pm0.26$ &   74. &$-1.85\pm0.31$ &   28. & \ldots & \ldots & \ldots & \ldots &$-1.80\pm0.28$ &   58. & \ldots & \ldots & \ldots & \ldots &$-1.75\pm0.28$ &   59. &$-1.80\pm0.24$ &   59. & \ldots & \ldots & \ldots & \ldots &$-1.60\pm0.25$ &   81. &$-2.00\pm0.22$ &   31. &$-1.75\pm0.26$ &   99. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.80\pm0.27$ &   75. &$-2.05\pm0.22$ &   56. &$-1.55\pm0.35$ &   60. & \ldots & \ldots &$-1.90\pm0.30$ &   47.\\
6575.020& 26.0& 2.588&$ -2.710$ & \ldots & \ldots &$-2.15\pm0.18$ &   73. & \ldots & \ldots &$-2.20\pm0.18$ &   32. & \ldots & \ldots & \ldots & \ldots &$-1.75\pm0.30$ &   70. &$-2.30\pm0.17$ &   46. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.70\pm0.26$ &   68. &$-1.85\pm0.31$ &   39. & \ldots & \ldots & \ldots & \ldots &$-2.05\pm0.28$ &   32. & \ldots & \ldots & \ldots & \ldots &$-1.75\pm0.28$ &   57. &$-1.80\pm0.24$ &   67. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.10\pm0.22$ &   35. &$-1.75\pm0.26$ &   91. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.70\pm0.33$ &   51. & \ldots & \ldots &$-1.70\pm0.30$ &   73. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.85\pm0.27$ &   66. &$-2.10\pm0.22$ &   56. & \ldots & \ldots & \ldots & \ldots &$-1.80\pm0.30$ &   69.\\
6592.910& 26.0& 2.727&$ -1.473$ & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.85\pm0.25$ &   43. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
6593.870& 26.0& 2.433&$ -2.422$ & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.70\pm0.22$ &   36. & \ldots & \ldots &$-2.31\pm0.21$ &   76. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.15\pm0.23$ &   60. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.18\pm0.25$ &   73. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
6608.020& 26.0& 2.279&$ -4.030$ & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.70\pm0.14$ &   50. & \ldots & \ldots &$-1.35\pm0.12$ &   44. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.80\pm0.13$ &   27. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.75\pm0.12$ &   31. & \ldots & \ldots &$-1.75\pm0.13$ &   28. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.70\pm0.15$ &  999. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
6609.110& 26.0& 2.559&$ -2.692$ & \ldots & \ldots &$-2.20\pm0.12$ &   95. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.80\pm0.12$ &   83. &$-2.20\pm0.12$ &   54. & \ldots & \ldots &$-1.80\pm0.13$ &   53. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.00\pm0.12$ &   56. &$-1.90\pm0.13$ &   60. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.95\pm0.12$ &   65. &$-2.00\pm0.12$ &   69. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.85\pm0.13$ &   69. &$-2.10\pm0.12$ &   47. & \ldots & \ldots & \ldots & \ldots &$-1.85\pm0.13$ &   70.\\
6703.570& 26.0& 2.758&$ -3.160$ &$-1.45\pm0.12$ &   58. &$-1.95\pm0.12$ &   52. & \ldots & \ldots & \ldots & \ldots &$-1.30\pm0.13$ &   58. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.35\pm0.12$ &   59. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.70\pm0.12$ &   32. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.55\pm0.12$ &   62. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.90\pm0.12$ &   26. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
6710.320& 26.0& 1.485&$ -4.880$ &$-1.60\pm0.12$ &   56. &$-1.95\pm0.12$ &   39. &$-1.60\pm0.12$ &   60. & \ldots & \ldots &$-1.45\pm0.13$ &   59. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.45\pm0.12$ &   55. & \ldots & \ldots & \ldots & \ldots &$-1.50\pm0.13$ &   64. & \ldots & \ldots & \ldots & \ldots &$-1.70\pm0.12$ &   39. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.75\pm0.12$ &   51. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
6739.520& 26.0& 1.557&$ -4.794$ &$-1.60\pm0.12$ &   32. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.60\pm0.17$ &   38. & \ldots & \ldots & \ldots & \ldots &$-1.50\pm0.13$ &   55. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
6750.150& 26.0& 2.424&$ -2.621$ & \ldots & \ldots &$-2.02\pm0.17$ &  105. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.20\pm0.12$ &   78. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.95\pm0.12$ &   61. & \ldots & \ldots & \ldots & \ldots &$-2.05\pm0.12$ &   52. & \ldots & \ldots &$-1.95\pm0.12$ &   91. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-2.05\pm0.12$ &   60. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.95\pm0.13$ &   82. &$-2.05\pm0.12$ &   67. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
6806.840& 26.0& 2.727&$ -3.210$ & \ldots & \ldots &$-2.00\pm0.12$ &   61. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.40\pm0.12$ &   58. & \ldots & \ldots & \ldots & \ldots &$-1.45\pm0.13$ &   67. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots &$-1.60\pm0.12$ &   54. & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots & \ldots \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\enddata 
\end{deluxetable}

